GuidedQuant: Large Language Model Quantization via Exploiting End Loss Guidance

Post-training quantization is a key technique for reducing the memory and inference latency of large language models by quantizing weights and activations without requiring retraining. However, existing methods either (1) fail to account for the varying importance of hidden features to the end loss or, when incorporating end loss, (2) neglect the critical interactions between model weights. To address these limitations, we propose GuidedQuant, a novel quantization approach that integrates gradient information from the end loss into the quantization objective while preserving cross-weight dependencies within output channels. GuidedQuant consistently boosts the performance of state-of-the-art quantization methods across weight-only scalar, weight-only vector, and weight-and-activation quantization. Additionally, we introduce a novel non-uniform scalar quantization algorithm, which is guaranteed to monotonically decrease the quantization objective value, and outperforms existing methods in this category. We release the code at https://github.com/snu-mllab/GuidedQuant.

==> figures/method.tex <==





\begin{figure*}
    \centering

\begin{tikzpicture}[
    2d-arr/.style={matrix of nodes, row sep=-\pgflinewidth, column sep=-\pgflinewidth, 
    nodes in empty cells,
    nodes={draw,
      minimum size=15pt,
      anchor=center,
      align=center,
      inner sep=0pt
    },}
  ]

  \matrix (W) [2d-arr] {
  |[fill=purple!40]| &  |[fill=purple!40]| &  |[fill=orange!40]| &  |[fill=orange!40]| & |[fill=pink!40]| &  |[fill=pink!40]| & |[fill=yellow!40]| & |[fill=yellow!40]| \\
  |[fill=purple!40]| &  |[fill=purple!40]| &  |[fill=orange!40]| &  |[fill=orange!40]| & |[fill=pink!40]| &  |[fill=pink!40]| & |[fill=yellow!40]| & |[fill=yellow!40]| \\
  |[fill=purple!40]| &  |[fill=purple!40]| &  |[fill=orange!40]| &  |[fill=orange!40]| & |[fill=pink!40]| &  |[fill=pink!40]| & |[fill=yellow!40]| & |[fill=yellow!40]| \\
  |[fill=purple!40]| &  |[fill=purple!40]| &  |[fill=orange!40]| &  |[fill=orange!40]| & |[fill=pink!40]| &  |[fill=pink!40]| & |[fill=yellow!40]| & |[fill=yellow!40]| \\
  };

  \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}] 
  ($(W-3-1.south west) + (0.2em, 0em)$) -- ($(W-3-3.south west) + (-0.2em, 0em)$) node[midway,yshift=-3em]{$J_1$};


  \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}] 
  ($(W-3-3.south west) + (0.2em, 0em)$) -- ($(W-3-5.south west) + (-0.2em, 0em)$) node[midway,yshift=-3em]{$J_2$};
  
  
  \node[below=1.0em of W-4-6.south west]{$\ldots$};
  
  
  \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}] 
  ($(W-3-7.south west) + (0.2em, 0em)$) -- ($(W-3-8.south east) + (-0.2em, 0em)$) node[midway,yshift=-3em]{$J_g$};


  \matrix (hW) [2d-arr, below=4em of W] {
  |[fill=purple!60!black!60]| &  |[fill=purple!60!black!60]| &  |[fill=orange!60!black!60]| &  |[fill=orange!60!black!60]| & |[fill=pink!20]|          &  |[fill=pink!60!black!60]| & |[fill=yellow!20]|          & |[fill=yellow!20]| \\
  |[fill=purple!20]|          &  |[fill=purple!60!black!60]| &  |[fill=orange!60!black!60]| &  |[fill=orange!60!black!60]| & |[fill=pink!20]|          &  |[fill=pink!60!black!60]| & |[fill=yellow!60!black!60]| & |[fill=yellow!20]| \\
  |[fill=purple!20]|          &  |[fill=purple!60!black!60]| &  |[fill=orange!60!black!60]| &  |[fill=orange!20]|          & |[fill=pink!20]|          &  |[fill=pink!60!black!60]| & |[fill=yellow!60!black!60]| & |[fill=yellow!20]| \\
  |[fill=purple!20]|          &  |[fill=purple!60!black!60]| &  |[fill=orange!20]|          &  |[fill=orange!20]|          & |[fill=pink!60!black!60]| &  |[fill=pink!60!black!60]| & |[fill=yellow!60!black!60]| & |[fill=yellow!60!black!60]| \\
  };
  
  
  \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}] 
  ($(hW-3-1.south west) + (0.2em, 0em)$) -- ($(hW-3-3.south west) + (-0.2em, 0em)$) node[midway,yshift=-3em]{$J_1$};


  \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}] 
  ($(hW-3-3.south west) + (0.2em, 0em)$) -- ($(hW-3-5.south west) + (-0.2em, 0em)$) node[midway,yshift=-3em]{$J_2$};
  
  
  \node[below=1.0em of hW-4-6.south west]{$\ldots$};
  
  
  \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}] 
  ($(hW-3-7.south west) + (0.2em, 0em)$) -- ($(hW-3-8.south east) + (-0.2em, 0em)$) node[midway,yshift=-3em]{$J_g$};
  
  
  \draw[dashed, black] ($(W-1-8.north east) + (1em, 2.5em)$) -- ($(hW-4-8.south east)+ (1em, -1.5em)$);
  
  \matrix (sal1) [2d-arr, right=4.3em of W] {
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  };
  
  \matrix (sal2) [2d-arr, right=4.3em of hW] {
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  |[fill=red!50]| \\
  };

 \node[left=0.7em of sal1-3-1,yshift=0.0em] {\large{$\mathrm{diag}$}}; 
 \node[left=0.7em of sal1-3-1,xshift=0.8em, yshift=0.0em] {$\left(\vphantom{\rule{2em}{1.5em}}\right.$};
 \node[left=0.2em of sal1-3-1,xshift=3.2em, yshift=0.0em] {$\left.\vphantom{\rule{2em}{1.5em}}\right)$};

 \node[left=0.7em of sal2-3-1,yshift=0.0em] {\large{$\mathrm{diag}$}}; 
 \node[left=0.7em of sal2-3-1,xshift=0.8em, yshift=0.0em] {$\left(\vphantom{\rule{2em}{1.5em}}\right.$};
 \node[left=0.2em of sal2-3-1,xshift=3.2em, yshift=0.0em] {$\left.\vphantom{\rule{2em}{1.5em}}\right)$};



  \node[above=-0.3em of W] {$\mathbf W \in \mathbb{R}^{d_\mathrm{in} \times d_\mathrm{out}}$};
  \node[above=-0.3em of hW] {$\widehat{\mathbf{W}} \in \mathbb{R}^{d_\mathrm{in} \times d_\mathrm{out}}$};


  \node[above=-0.3em of sal1] {$\mathbf{s}_1 \in \mathbb{R}^{n\times 1}$};
  \node[above=-0.3em of sal2] {$\mathbf{s}_g \in \mathbb{R}^{n\times 1}$};
  \node[above=1.15em of sal2] {$\vdots$};
 
    

  \node[right=0.9em of sal1] (str) {\Large{$\ast$}};
  \node[right=0.9em of sal2] (str2) {\Large{$\ast$}};


  \matrix (X) [2d-arr, right=0.2em of str, nodes={draw, fill=lightgray!30}] {
    &  &  & \\
    &  &  & \\
    &  &  & \\
    &  &  & \\
    &  &  & \\
  };
  
  
  \matrix (X2) [2d-arr, right=0.2em of str2, nodes={draw, fill=lightgray!30}] {
    &  &  & \\
    &  &  & \\
    &  &  & \\
    &  &  & \\
    &  &  & \\
  };
%   \node[below=of K-3-2] {$\mathbf K$};

  \node[right=0.2em of X] (eq) {\Large{$\ast$}};
 \node[right=0.2em of X2] (eq2) {\Large{$\ast$}};

  \matrix (lw1) [2d-arr, right=1.0em of eq] {
 |[fill=purple!60!black!60]| &  |[fill=purple!60!black!60]| \\
 |[fill=purple!20]|          &  |[fill=purple!60!black!60]| \\
 |[fill=purple!20]|          &  |[fill=purple!60!black!60]| \\
 |[fill=purple!20]|          &  |[fill=purple!60!black!60]| \\
  };
 \matrix (lw2) [2d-arr, right=1.0em of eq2] {
 |[fill=yellow!20]|          & |[fill=yellow!20]| \\
 |[fill=yellow!60!black!60]| & |[fill=yellow!20]| \\
 |[fill=yellow!60!black!60]| & |[fill=yellow!20]| \\
 |[fill=yellow!60!black!60]| & |[fill=yellow!60!black!60]| \\
  };
  

 \node[right=0.0em of lw1] (eq) {\Large{$-$}};
 \node[right=0.0em of lw2] (eq2) {\Large{$-$}};
  
  
  
 \node[left=0.5em of lw1,xshift=1.0em, yshift=0.0em] {$\left(\vphantom{\rule{2em}{2em}}\right.$};
 \node[left=0.5em of lw1,xshift=11.0em, yshift=0.0em] {$\left.\vphantom{\rule{2em}{2em}}\right)$};

  
 \node[left=0.5em of lw2,xshift=1.0em, yshift=0.0em] {$\left(\vphantom{\rule{2em}{2em}}\right.$};
 \node[left=0.5em of lw2,xshift=11.0em, yshift=0.0em] {$\left.\vphantom{\rule{2em}{2em}}\right)$};


  \matrix (rw1) [2d-arr, right=1.8em of lw1] {
|[fill=purple!40]| &  |[fill=purple!40]| \\
|[fill=purple!40]| &  |[fill=purple!40]| \\
|[fill=purple!40]| &  |[fill=purple!40]| \\
|[fill=purple!40]| &  |[fill=purple!40]|\\
  };
 \matrix (rw2) [2d-arr, right=1.8em of lw2] {
|[fill=yellow!40]| & |[fill=yellow!40]| \\
|[fill=yellow!40]| & |[fill=yellow!40]| \\
|[fill=yellow!40]| & |[fill=yellow!40]| \\
|[fill=yellow!40]| & |[fill=yellow!40]| \\
  };

  \node[above=-0.3em of rw1] {$\mathbf{W}\left[:, J_1\right]$};
  \node[above=-0.3em of rw2] {$\mathbf{W}\left[:, J_g\right]$};
  \node[above=2.0em of rw2] {$\vdots$};


  \node[above=-0.3em of lw1] {$\widehat{\mathbf{W}}\left[:, J_1\right]$};
  \node[above=-0.3em of lw2] {$\widehat{\mathbf{W}}\left[:, J_g\right]$};
  \node[above=2.0em of lw2] {$\vdots$};


  \node[above=-0.3em of X] {$\mathbf{X}\in\mathbb{R}^{n \times d_\mathrm{in}}$};
  \node[above=-0.3em of X2] {$\mathbf{X}\in\mathbb{R}^{n \times d_\mathrm{in}}$};


\draw[->] ($(rw1-2-2.south east) + (1.5em, 0em)$) to[out=0, in=110]  ($(rw1-2-2.south east) + (5.0em, -3.0em)$);
\node[right=4em of rw1-3-2] {$(\;\cdot\;)^2$};


\draw[->] ($(rw2-2-2.south east) + (1.5em, 0em)$) to[out=0, in=250]  ($(rw2-2-2.south east) + (5.0em, 3.0em)$);
\node[right=4em of rw2-2-2] (ds) {$(\;\cdot\;)^2$};

\node[above=4em of ds] {Minimize the};
\node[above=3em of ds] {sum of};
\node[above=1.8em of ds] {squared error};



  
%   \node[below=of ret-4-3] {$\mathbf{I * K}$};

%   \draw[dashed, teal] (mtr-1-6.north east) -- (K-1-1.north west);
%   \draw[dashed, teal] (mtr-3-6.south east) -- (K-3-1.south west);

%   \draw[dashed, blue!80!black] (K-1-3.north east) -- (ret-1-4.north west);
%   \draw[dashed, blue!80!black] (K-3-3.south east) -- (ret-1-4.south west);

%   \foreach \i in {1,2,3} {
%       \foreach \j in {4,5,6} {
%           \node[font=\tiny, scale=0.6, shift={(-1.2ex,-2ex)}] at (mtr-\i-\j) {$\times \pgfmathparse{int(mod(\i+\j,2))}\pgfmathresult$};
%         }
%     }

\end{tikzpicture}

    \caption{An illustration of GuidedQuant method quantizing a single linear layer. We denote input, weight, and the quantized weight as $\bX \in \mathbb{R}^{n \times d_\mathrm{in}}$, $\hat{\mathbf{W}}\in\mathbb{R}^{d_\mathrm{in} \times d_\mathrm{out}}$, and $\mathbf{W}\in\mathbb{R}^{d_\mathrm{in} \times d_\mathrm{out}}$, respectively. $J_1, \ldots, J_g$ represent a partition of the index set $\{1, \ldots, d_\mathrm{out}\}$. $\mathbf{s}_k$ is calculated through the root mean square of the gradient within the $k$-th group of output features, $\frac{1}{\lvert J_k \rvert} \sum_{j\in J_k} \frac{\partial \ell}{\partial (\bX \bW[}$ GuidedQuant method minimizes the reconstruction error weighted by the average gradient information }
    \label{fig:qual2}
\end{figure*}


==> tables/group_backup.tex <==
\begin{table*}[t]
\caption{Results with different number of groups $g$ in weight-only post-training quantization results on non-uniform scalar quantization format, \textit{without fine-tuning} to the end-to-end loss. Wiki2 and C4 denotes perplexity on WikiText2 and C4, respectively, which are measured with the context size of 4096.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=1.7\columnwidth}
\begin{tabular}{lc ccc ccc ccc}
\toprule
& \multirow{2}{*}{Number of} & \multicolumn{3}{c}{Llama-2-7B} & \multicolumn{3}{c}{Llama-2-13B} & \multicolumn{3}{c}{Llama-2-70B} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Method &
groups $g$ & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$  \\
\cmidrule(lr){1-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}\cmidrule(lr){7-8}\cmidrule(lr){9-9}\cmidrule(lr){10-11}
% \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Original & -- &
16 & 5.12 & 6.63 &  %& 
16 & 4.57 & 6.05 &  %& 
16 & 3.12 & 4.97 \\%&  \\
\cmidrule(lr){1-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}\cmidrule(lr){7-8}\cmidrule(lr){9-9}\cmidrule(lr){10-11}
LNQ & -- &
2.01 & 22.49 & 25.37 &  %& 
2.01 & 8.96  & 11.97 &  %& 
2.01 & 5.52 & 7.61\\%&  \\
LNQ + GuidedQuant & 1 & 
2.01 & 9.27 & 11.30 &  
2.01 & 7.28 & 9.28 & 
2.01 & 5.40 & 7.40\\ 
 & 2 & 
2.01 & 8.68 & 11.20 &  
2.01 & 7.30 & 9.28 & 
2.01 & 5.30 & 7.39 \\ 
 & 4 & 
2.01 & 8.84 & 11.09 &  
2.01 & 7.19 & 9.24 & 
-- & -- & -- \\ 
\cmidrule(lr){1-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}\cmidrule(lr){7-8}\cmidrule(lr){9-9}\cmidrule(lr){10-11}
LNQ  & -- & 
3.03 & 5.91 & 7.78 &  %& 
3.02 & 5.03 & 6.69 &  %& 
3.01 & 3.52 & 5.32\\%&  \\
LNQ + GuidedQuant & 1 & 
3.03 & 5.57 & 7.23 &  
3.02 & 4.92 & 6.49 & 
3.01 & 3.49 & 5.29 \\ 
 & 2 & 
3.03 & 5.55 & 7.22 &  
3.02 & 4.92 & 6.49 & 
3.01 & 3.49 & 5.29 \\ 
 & 4 & 
3.03 & 5.55 & 7.22 &  
3.02 & 4.91 & 6.49 & 
-- & -- & -- \\ 
\cmidrule(lr){1-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}\cmidrule(lr){6-6}\cmidrule(lr){7-8}\cmidrule(lr){9-9}\cmidrule(lr){10-11}
LNQ  & -- & 
4.05  & 5.27 & 6.82 &  %& 
4.04  & 4.68 & 6.17 &  %& 
4.03 & 3.20 & 5.04\\%&  \\
LNQ + GuidedQuant & 1 & 
4.05 & 5.21 & 6.75 &  
4.04 & 4.65 & 6.14 & 
4.03 & 3.21 & 5.03\\ 
 & 2 & 
4.05 & 5.22 & 6.75 &  
4.04 & 4.65 & 6.14 & 
4.03 & 3.20 & 5.03 \\ 
 & 4 & 
4.05 & 5.21 & 6.75 &  
4.04 & 4.65 & 6.14 & 
-- & -- & -- \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:group}
\end{table*}


==> tables/wa_ppl.tex <==

\begin{table*}[t]
\caption{Weight-and-activation quantization results on Llama-2 models.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{c l cc cc cc}
\toprule
& & \multicolumn{2}{c}{Llama-2-7B} & \multicolumn{2}{c}{Llama-2-13B} & \multicolumn{2}{c}{Llama-2-70B} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
% & \multicolumn{2}{c}{Llama-2-7B} & \multicolumn{2}{c}{Llama-2-13B} & \multicolumn{2}{c}{Llama-2-70B} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Bits & Method &  
Acc$\uparrow$($\%$) & 
Wiki2$\downarrow$ &  
Acc$\uparrow$($\%$) & 
Wiki2$\downarrow$ &  
Acc$\uparrow$($\%$) & 
Wiki2$\downarrow$ 
\\
% \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
% \cmidrule(lr){1-2}\cmidrule{3-4}\cmidrule(lr){5-6}\cmidrule{7-8}
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
16& FP16 & & 5.47 & & 4.88 \\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
\multirow{3}{*}{\shortstack[c]{W4A4KV4}}
&QuaRot & & 6.08 & & 5.39
\\
&SpinQuant & & 5.94 & & 5.25
\\
&SpinQuant + GQuant (Ours) & & \textbf{5.89} & & \textbf{5.20}
\\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
\multirow{3}{*}{\shortstack[c]{W4A4KV16}}
&QuaRot & & 6.02 & & 5.34
\\
&SpinQuant & & 5.90 & & 5.21
\\
&SpinQuant + GQuant (Ours) & & \textbf{5.84} & & \textbf{5.17}
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:wa}
\end{table*}

==> tables/wo_h_ppl_v1.tex <==

\begin{table*}[t]
\caption{Weight-only high-dimensional quantization results.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{Llama-2-7B} & \multicolumn{3}{c}{Llama-2-13B} & \multicolumn{3}{c}{Llama-2-70B} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Method & 
Bits $\downarrow$ & 
Wiki2 $\downarrow$ & 
C4 $\downarrow$ & 
Bits $\downarrow$ & 
Wiki2 $\downarrow$ & 
C4 $\downarrow$ & 
Bits $\downarrow$ & 
Wiki2 $\downarrow$ & 
C4 $\downarrow$ \\
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
GPTVQ                     &  &  &  &  &  &  &  &  &   \\
QuIP\#                     &  &  &  &  &  &  &  &  &   \\
AQLM                      &  &  &  &  &  &  &  &  &   \\
QTIP                      &  &  &  &  &  &  &  &  &   \\
QTIP + GQuant (Ours)     &  &  &  &  &  &  &  &  &   \\
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
GPTVQ                     &  &  &  &  &  &  &  &  &   \\
QuIP\#                     &  &  &  &  &  &  &  &  &   \\
AQLM                      &  &  &  &  &  &  &  &  &   \\
QTIP                      &  &  &  &  &  &  &  &  &   \\
QTIP + GQuant (Ours)     &  &  &  &  &  &  &  &  &   \\
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
GPTVQ                     &  &  &  &  &  &  &  &  &   \\
QuIP\#                     &  &  &  &  &  &  &  &  &   \\
AQLM                      &  &  &  &  &  &  &  &  &   \\
QTIP                      &  &  &  &  &  &  &  &  &   \\
QTIP + GQuant (Ours)     &  &  &  &  &  &  &  &  &   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:rn34}
\end{table*}

==> tables/wo_h_ppl_v2.tex <==
\begin{table*}[t]
\caption{Weight-only high-dimensional quantization results.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{l cccc cccc cccc}
\toprule
& \multicolumn{4}{c}{Llama-2-7B} & \multicolumn{4}{c}{Llama-2-13B} & \multicolumn{4}{c}{Llama-2-70B} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Method & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Tok/s$\uparrow$ &
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Tok/s$\uparrow$ &
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ &
Tok/s$\uparrow$ \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
FP16 & 
16 & 5.12 & 6.63 &  & 
16 & 4.57 & 6.05 &  & 
16 & 3.12 & 4.97 &  \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
GPTVQ 2D&
2.13 & 10.66 & 12.81 & -- & 
2.13 & 7.55 & 9.82 & -- & 
2.13 & 5.06 & 7.09 & -- \\
GPTVQ 4D&
2.25 & 7.89 & 10.25 & -- & 
2.25 & 6.36 & 8.43 & -- & 
2.25 & 4.44 & 6.28 & -- \\
QuIP\# &
2.00 & 8.22 & 11.01 &  & 
2.00 & 6.06 & 8.07 &  & 
2.00 & 4.16 & 6.01 &  \\
AQLM & 
2.02 & 6.59 & 8.54 &  & 
2.19 & 5.37 & 7.16 &  & 
2.07 & 3.94 & 5.72 &  \\
QTIP & 
2.00 & 6.82 & 8.96 &  & 
2.00 & 5.52 & 7.39 &  & 
2.00 & 3.87 & 5.69 &  \\
QTIP + GQuant (Ours) & 
2.00 & \textbf{6.11} & \textbf{7.99} &  & 
2.00 & \textbf{5.33} & \textbf{7.05} &  & 
2.00 &  &  &  \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
GPTVQ 2D&
3.13 & 5.63 & 7.32 & -- & 
3.13 & 4.87 & 6.45 & -- & 
3.13 & 3.38 & 5.18 & -- \\
QuIP\# & 
3.00 & 5.60 & 7.34 &  & 
3.00 & 4.90 & 6.50 &  & 
3.00 & 3.41 & 5.20 &  \\
AQLM & 
3.04 & 5.46 & 7.08 &  & 
3.03 & 4.82 & 6.37 &  & 
3.01 & 3.36 & 5.17 &  \\
QTIP & 
3.00 & 5.38 & 6.99 &  & 
3.00 & 4.74 & 6.28 &  & 
3.00 & 3.27 & 5.09 &  \\
QTIP + GQuant (Ours) & 
3.00 & \textbf{5.28} & \textbf{6.87} &  & 
3.00 & \textbf{4.71} & \textbf{6.22} &  & 
3.00 &  &  &  \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
GPTVQ 2D&
4.13 & 5.24 & 6.77 & -- & 
4.13 & 4.65 & 6.13 & -- & 
4.13 &  &  & -- \\
QuIP\# & 
4.00 & 5.22 & 6.79 &  & 
4.00 & 4.65 & 6.15 &  & 
4.00 & 3.18 & 5.02 &  \\
AQLM & 
4.04 & 5.21 & 6.75 &  & 
3.94 & 4.65 & 6.14 &  & 
4.14 & 3.19 & 5.03 &  \\
QTIP & 
4.00 & 5.17 & 6.71 &  & 
4.00 & 4.62 & 6.10 &  & 
4.00 & 3.16 & 5.00 &  \\
QTIP + GQuant (Ours) & 
4.00 & \textbf{5.16} & \textbf{6.68} &  & 
4.00 & \textbf{4.61} & \textbf{6.09} &  & 
4.00 &  &  &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:rn34}
\end{table*}


==> tables/wo_s_ppl_v1.tex <==

\begin{table*}[t]
\caption{Weight-only scalar quantization results.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{Llama-2-7B} & \multicolumn{3}{c}{Llama-2-13B} & \multicolumn{3}{c}{Llama-2-70B} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Method & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ \\
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
FP16                      & 16 & 5.12 & 6.63 & 16 & 4.57 & 6.05  & 16 & 3.12 &  4.97  \\
AWQ                       &  &  &  &  &  &  &  &  &   \\
OmniQuant                 &  &  &  &  &  &  &  &  &   \\
QuIP                      & -- & -- & -- & 2.00 & 13.48 & 16.16 & 2.00 & 5.90 &  8.17  \\
SqueezeLLM                & 2.01 & 39.58 & 44.05 & 2.01 & 16.24 & 19.20 & 2.01 & 9.17 &  13.03 \\
GPTVQ 1D                  & 2.13 &  &   & 2.13 &  &  & 2.13 &  &   \\
GNQ + GQuant (Ours)       & 2.01 &  &   & 2.01 &  &  & 2.01 &  &   \\
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
GPTQ                      &  &  &  &  &  &  &  &  &   \\
AWQ                       &  &  &  &  &  &  &  &  &   \\
OmniQuant                 &  &  &  &  &  &  &  &  &   \\
QuIP                      &  &  &  &  &  &  &  &  &   \\
SqueezeLLM                &  &  &  &  &  &  &  &  &   \\
GPTVQ 1D                  &  &  &  &  &  &  &  &  &   \\
GNQ + GQuant (Ours) &  &  &  &  &  &  &  &  &   \\
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
GPTQ                      &  &  &  &  &  &  &  &  &   \\
AWQ                       &  &  &  &  &  &  &  &  &   \\
OmniQuant                 &  &  &  &  &  &  &  &  &   \\
QuIP                      &  &  &  &  &  &  &  &  &   \\
SqueezeLLM                &  &  &  &  &  &  &  &  &   \\
GPTVQ 1D                  &  &  &  &  &  &  &  &  &   \\
GNQ + GQuant (Ours) &  &  &  &  &  &  &  &  &   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:scalar}
\end{table*}

==> tables/wo_s_ppl_v2.tex <==

\begin{table*}[t]
\caption{Weight-only scalar quantization results.}
\vspace{0.5em}
\centering
\begin{adjustbox}{max width=2.0\columnwidth}
\begin{tabular}{l cccc cccc cccc}
\toprule
& \multicolumn{4}{c}{Llama-2-7B} & \multicolumn{4}{c}{Llama-2-13B} & \multicolumn{4}{c}{Llama-2-70B} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
Method & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ & 
Tok/s$\uparrow$ & 
Bits$\downarrow$ & 
Wiki2$\downarrow$ & 
C4$\downarrow$ &
Tok/s$\uparrow$ &
Bits$\downarrow$ & 
Wiki2$\downarrow$ &
C4$\downarrow$ &
Tok/s$\uparrow$ \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
FP16 & 
16 & 5.12 & 6.63 &  & 
16 & 4.57 & 6.05 &  & 
16 & 3.12 & 4.97 & OOM \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
% AWQ & 
%  &  &  &  & 
%  &  &  &  & 
%  &  &  &  \\
% OmniQuant & 
%  &  &  &  & 
%  &  &  &  & 
%  &  &  &  \\
QuIP & 
-- & -- & -- & -- & 
2.00 & 13.48 & 16.16 &  &
2.01 & 5.90 & 8.17 &  \\
SqueezeLLM & 
2.01 & 39.58 & 44.05 &  &
 & 16.24 & 19.20 &  &
 & 9.17 & 13.03 &  \\
GPTVQ 1D & 
2.13 & 14.61 & 16.95 & -- & 
2.13 & 8.39 & 11.20 & -- &
% 2.13 & 5.20 & 7.39 & -- \\
\\
LNQ + GQuant (Ours) & 
2.01 & \textbf{8.92} & \textbf{11.15} &  & 
 & \textbf{7.27} & \textbf{9.33} &  &
 & \textbf{5.33} & \textbf{7.39} &  \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
GPTQ & 
3.00 & 8.06 & 10.61 &  & 
3.00 & 5.85 &  7.86 &  & 
3.00 & 4.40 &  6.26 &  \\
% AWQ & 
%  &  &  &  & 
%  &  &  &  & 
%  &  &  &  \\
% OmniQuant & 
%  &  &  &  & 
%  &  &  &  & 
%  &  &  &  \\
QuIP & 
-- & -- & -- & -- & 
3.00 & 5.12 &  6.79 &  & 
3.01 & 3.87 &  5.67 &  \\
SqueezeLLM & 
3.02 & 5.74 & 7.44 &  & 
 & 4.99 & 6.60 &  &
 & 3.53 & 5.31 &  \\
GPTVQ 1D & 
3.13 & 5.93 & 7.73 &  & 
3.13 & 5.05 & 6.67 &  & 
% 3.13 & 3.50 & 5.29 &  \\
\\
LNQ + GQuant (Ours) & 
3.02 & \textbf{5.57} & \textbf{7.22} &  & 
 & \textbf{4.91} & \textbf{6.49} &  & 
 & \textbf{3.49} & \textbf{5.29} &  \\
\cmidrule(lr){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
GPTQ & 
4.00 & 5.49 & 7.20 &  & 
4.00 & 4.78 & 6.34 &  & 
4.00 & 3.35 & 5.15 &  \\
% AWQ & 
%  &  &  &  & 
%  &  &  &  & 
%  &  &  &  \\
% OmniQuant & 
%  &  &  &  & 
%  &  &  &  & 
%  &  &  &  \\
QuIP & 
 -- & -- & -- & -- & 
 4.00 & 4.76 & 6.29 &  & 
 4.00 & 3.58 &  5.38 &  \\
SqueezeLLM & 
4.05 & 5.23 & 6.78 &  & 
 & 4.67 & 6.15 &  & 
 & \textbf{3.20} & 5.04 &  \\
GPTVQ 1D & 
4.13 & 5.28 & 6.81 &  & 
4.13 & 4.66 & 6.15 &  & 
% 4.13 & 3.19 & 5.02 &  \\
\\
LNQ + GQuant (Ours) & 
4.05 & \textbf{5.21} & \textbf{6.75} &  & 
 & \textbf{4.65} & \textbf{6.14} &  & 
 & \textbf{3.20} & \textbf{5.03} &  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:scalar}
\end{table*}
